Disentangled Speech Embeddings using Cross-modal Self-supervision

The objective of this paper is to learn representations of speaker identity without access to manually annotated data. To do so, we develop a self-supervised learning objective that exploits the natural cross-modal synchrony between faces and audio in video. The key idea behind our approach is to tease apart--without annotation--the representations of linguistic content and speaker identity. We construct a two-stream architecture which: (1) shares low-level features common to both representations; and (2) provides a natural mechanism for explicitly disentangling these factors, offering the potential for greater generalisation to novel combinations of content and identity and ultimately producing speaker identity representations that are more robust. We train our method on a large-scale audio-visual dataset of talking heads `in the wild', and demonstrate its efficacy by evaluating the learned speaker representations for standard speaker recognition performance.

==> resnet.tex <==
\begin{table}[ht]
\footnotesize
\centering
\begin{tabular}{ c|c|c }
\textbf{layer name} & \textbf{VGG-M-40}  & \textbf{Thin ResNet-34}   \\ \hline
conv1 & \makecell{$5 \times 7,96$, st. 2 \\ $ 3 \times 3$, max pool, st. $ 1 \times 2$}  & \makecell{$7 \times 7,16$, st. 2 \\ $ 3 \times 3$, max pool, st. 2}  \\   \hline
%\addlinespace[1.5ex]
conv2 &  \makecell{$5 \times 5,96$, st. 2 \\ $ 3 \times 3$, max pool, st. 2}    & $\begin{bmatrix}  3 \times 3, 16 \\ 3 \times 3, 16 \end{bmatrix} \times 3 $, st. 1         \\\hline
%\addlinespace[1.5ex]
conv3 & $3 \times 3,256$, st. 1 & $\begin{bmatrix}  3 \times 3,32 \\ 3 \times 3,32 \end{bmatrix} \times 4 $, st. 2      \\\hline
%\addlinespace[1.5ex]
conv4 & $3 \times 3,256$, st. 1 & $\begin{bmatrix}  3 \times 3,64 \\ 3 \times 3,64 \end{bmatrix} \times 6 $, st. 2        \\\hline
%\addlinespace[1.5ex]
conv5 &  \makecell{$3 \times 3,256$, st. 1 \\ $ 3 \times 3$, max pool, st. 2}    & $\begin{bmatrix}  3 \times 3,128 \\ 3 \times 3,128 \end{bmatrix} \times 3 $, st. 2       \\\hline
%\addlinespace[1.5ex]
fc &  $ 4 \times 1$, 512, st. 1  &  $ 9 \times 1$, 512, st. 1                  \\ 
\end{tabular}
\vspace{2pt}
\normalsize
\caption{Modified VGG-M and ResNet architectures. ReLU and batchnorm layers are not shown.  Each row specifies the number of convolutional filters, their sizes and strides as {\bf size $\times$ size, \# filters, stride}. The output from the fully connected layer is ingested by the pooling layers.}
\label{table:convnet}
\end{table}

==> results.tex <==
\begin{table*}[] 
\begin{center}
\footnotesize
\begin{tabular}{ |c | c | c | r | r | r|r|r|r| } 
 \hline
 \textbf{Model} &
 \textbf{Pooling} &
 \textbf{MVN}  &
 \textbf{Alpha} &
 \textbf{Iden. T1} &
 \textbf{Iden. T5} &
 \textbf{Ver. EER} &
 \textbf{Env. EER}
 \\ \hline
 VGG-M~\cite{Nagrani17} & TAP & \cmark &
           0 & - & - & 7.82\% & - \\ \hline
   \multirow{4}{50pt}{VGG-M-40} & \multirow{4}{30pt}{~~TAP} & \multirow{4}{30pt}{~~~~\cmark} &
           0 & 67.62\% & 82.90\% & 8.44\% & {\bf 18.72\%} \\ 
    & &  & 1 & 72.74\% & 87.15\% & 8.15\% & 20.01\% \\
    & &  & 10 & 75.96\% & 89.48\% & 7.79\% & 21.93\% \\
    & &  & 30 & {\bf 77.70\%} & {\bf 90.29\%} & {\bf 7.61\%} &  23.87\% \\\hline
   \multirow{4}{50pt}{VGG-M-40} & \multirow{4}{30pt}{~~SAP} & \multirow{4}{30pt}{~~~~\cmark} &
           0 & 68.13\% & 83.67\% & 8.02\% & {\bf 18.45\%} \\ 
    & &  & 1 & 70.99\% & 85.64\% & 8.31\% & 18.98\% \\
    & &  & 10 & 76.01\% & 89.53\% & 7.93\% & 21.63\% \\
    & &  & 30 & {\bf 77.31\%} & {\bf 90.48\%} & {\bf 7.82\%} & 23.55\% \\\hline
   \multirow{4}{70pt}{~Thin ResNet-34} & \multirow{4}{30pt}{~~SAP} & \multirow{4}{30pt}{~~~~\xmark} &
           0 & 67.58\% & 82.30\% & 8.28\% & {\bf 15.39\%} \\ 
    & &  & 1 & 75.71\% & 88.14\% & 7.73\% & 17.92\% \\
    & &  & 10 & 80.58\% & 91.98\% & 7.04\% & 20.77\% \\
    & &  & 30 & {\bf 81.45\%} & {\bf 92.66}\% & {\bf 6.59\%} &  21.70\% \\\hline
   \multirow{4}{70pt}{~Thin ResNet-34} & \multirow{4}{30pt}{~~SAP} & \multirow{4}{30pt}{~~~~\cmark} &
           0 & 83.68\% & 92.90\% & 5.71\% & {\bf 20.43\%} \\ 
    & &  & 1 & 88.34\% & 85.48\% & 5.38\% & 23.04\% \\
    & &  & 10 & {\bf 89.00\%} & 95.94\% & {\bf 5.26}\% & 25.74\% \\
    & &  & 30 & {\bf 89.00\%} & {\bf 96.15\%} & 5.37\% & 26.38\% \\\hline
\end{tabular}
\end{center}
\caption{
Results on speaker identification and verification tasks. Models for both tasks have been trained only on VoxCeleb1. Speaker identification is a 1,211-way classification task, excluding the 40 test set speakers.
Note that the scenario is different from~\cite{Nagrani17}, which trains the model for a 1,251-way classification task including the 40 test set speakers.
}
\normalsize
\label{tab:results}
\end{table*}
